Distributed Marker Representation for Ambiguous Discourse Markers and Entangled Relations

Discourse analysis is an important task because it models intrinsic semantic structures between sentences in a document. Discourse markers are natural representations of discourse in our daily language. One challenge is that the markers as well as pre-defined and human-labeled discourse relations can be ambiguous when describing the semantics between sentences. We believe that a better approach is to use a contextual-dependent distribution over the markers to express discourse information. In this work, we propose to learn a Distributed Marker Representation (DMR) by utilizing the (potentially) unlimited discourse marker data with a latent discourse sense, thereby bridging markers with sentence pairs. Such representations can be learned automatically from data without supervision, and in turn provide insights into the data itself. Experiments show the SOTA performance of our DMR on the implicit discourse relation recognition task and strong interpretability. Our method also offers a valuable tool to understand complex ambiguity and entanglement among discourse markers and manually defined discourse relations.

==> sections/04exp-dis.tex <==
\section{Experiments \& Discussion}
\label{sec:exp}

% DMR focuses on refining PLMs to obtain commonsense by modeling the latent discourse relations concealed by markers in sentence pairs. We first report its performance of marker prediction and then investigate the property of the latent space (Sec.~\ref{sec:exp:diagnostic}). Next, we verify its commonsense capability on commonsense required inference tasks (Sec.~\ref{sec:exp:commonsense}). 
% Finally, we report its capability to study discourse analysis and the insights we obtained.

DMR adopts a latent bottleneck for the space of latent discourse senses. We first prove the effectiveness of the latent variable and compare our framework to current SOTA solutions. We carefully investigate what the latent bottleneck learned during training and how it addresses the ambiguity and entanglement of discourse markers and relaitons.

\subsection{Set-up}
\label{sec:exp:setup}
Our DMR model is trained on Discovery data~\cite{sileo2019mining} with 1.74 million examples and 174 markers included. The sentence encoder is a baseline pretrained RoBERTa model~\cite{liu2019roberta}, which we call $\text{BASE}$, and is used as \texttt{SentEnc} in DMR. We set the default $K$ to 30. In all experiments, the encoders are instantiated as in baselines for a fair comparison. We leave details of task-specific settings in each section.
More details regarding the implementation of DMR can be found in Appendix~\ref{supp:implementation}.

We perform analysis on discourse relations by using the PDTB2~\cite{prasad2008penn} benchmark. We apply the typical level-2 11-way classification taxonomy with accuracy and macro-f1 scores as evaluation metrics. We follow~\cite{ji2015one} for data split, which is widely used in recent studies for IDRR. We note that although annotators are allowed to annotate multiple senses (relations), only 2.3\% of the data have more than one relation. Therefore whether DMR can capture more entanglement among relations is of interest as well.

For the IDRR task, we strip the marker generation part from the DMR model and use the hidden state $h_z$ as the pair representation.
$\text{BASE}$ uses the \texttt{[CLS]} token representation as the representation of input pairs.
A linear classification layer is stacked on top of models to predict relations. We also compare DMR to current SOTAs.

\input{tables/discourse}

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figs/fewshot_curve.pdf}
    \caption{Few-shot Implicit Discourse Relation Prediction}
    \label{fig:discourse}
\end{figure}

\input{tables/discourse-few.tex}

\subsection{Main Results on IDRR}
% More analysis here on the mdoel without a latent bottleneck.

We list the comparison to current SOTAs in Table~\ref{tab:discourse_relation_comp}. Despite its simple architecture, DMR leads in terms of accuracy by 2.5pt and is a close second in micro-F1.

Fig.~\ref{fig:discourse} shows DMV achieves significant gains against BASE in few-shot learning experiments. The results are averaged on 3 independent runs for each setting. In fact, with only $\sim$60\% of annotated data, DMV achieves the same performance as BASE with full data. This indicates that DVM has effectively utilized the cheap marker data.

To understand the ceiling of the family of such BERT-based pretrained model with markers as an extra input, we augment the data in two ways: $\text{BASE}_g$ inserts the groundtruth marker, and $\text{BASE}_p$ where the markers are predicted by a model\footnote{They also use the RobERTa model as a backbone.} officially released by Discovery~\cite{sileo2019mining}.
Table~\ref{tab:discourse_relation} presents the results where the informative markers are inserted to improve the performance of BASE, following the observations and ideas from ~\cite{zhou-etal-2010-predicting, pitler2008easily}. DMV continues to enjoy the lead, even when the markers are groundtruth (i.e. $\text{BASE}_g$), suggesting DMV's hidden state contains more information than markers.

% We also compare DMR against BASE in few-shot learning experiments. DMR achieves the same performance as BASE with only $\sim$60\% of annotated data.
% DMR continues to enjoy the lead, even when we insert groundtruth markers as a data augmentation to BASE. We refer the readers to Appendix~\ref{supp:discourse} for more details. 
The results exhibits the strength of DMR by more straightforwardly modeling the correlation between discourse markers and relations.

\dyru{comparison with Discovery model on full setting}

\subsection{Fine-grained Analysis on IDRR}
\input{tables/discourse-fine}


\subsection{Marker Prediction and Latent Space Analysis}
\label{sec:exp:diagnostic}

\paragraph{Marker Prediction} The performance of DMR on the pretraining marker prediction is sensitive to the capacity of the bottleneck. When setting $K$ to be the number of markers (174), it matches and even outperforms the Discovery model which directly predicts the markers on the same data (Table~\ref{tab:marker-prediction})\footnote{More analysis regarding the performance can be found in Appendix~\ref{supp:marker-ambiguity}.}. A smaller $K$ sacrifices marker prediction performance but it can cluster related senses, resulting in more informative and interpretable representation.

Multiple markers may share similar meanings when connecting sentences. Thus, evaluating the performance of marker prediction simply on top1 accuracy is inappropriate. In Table~\ref{tab:marker-prediction}, we demonstrated the results on ACC@k and observed that DMV(K=174) gets better performance against the model optimized by an MLE objective when k gets larger. We assume that it comes from the marker ambiguity. Our DMV models the ambiguity better, thus with any of the plausible markers easier to be observed in a larger range of predictions but more difficult as top1. To prove the marker ambiguity more directly, we randomly sample 50 examples to analyze their top5 predictions. The statistics show that over 80\% of those predictions have plausible explanations. To conclude, considerable examples have multiple plausible markers thus ACC@k with larger k can better reflect the true performance on marker prediction, where DMV can beat the MLE-optimized model.

\input{tables/diagnosis}


\paragraph{\emph{z2m} Mapping Analysis}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figs/tsne-crop.pdf}
%     \caption{The cropped T-SNE visualization of latent $\bm{z}$, each $\bm{z}$ is coupled with its top 3 markers from \emph{z2m} mapping.}
%     \label{fig:tsne-crop}
% \vspace{-10pt}
% \end{figure}

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.8\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/plm-tsne-crop.pdf}
         \caption{The cropped T-SNE visualization of discourse markers from the BASE PLM}
         \label{fig:plm-tsne-crop}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/tsne-crop.pdf}
         \caption{The cropped T-SNE visualization of latent $\bm{z}$ from DMR}
         \label{fig:dmr-tsne-crop}
    \end{subfigure}
    \caption{The cropped T-SNE visualization of latent $\bm{z}$ from DMR. Each $\bm{z}$ is coupled with its top 3 markers from \emph{z2m} mapping.}
    \label{fig:tsne-crop}
\end{figure}

The latent space is not interpretable, but DMR has a transition matrix that outputs a distribution of markers, which offers a glimpse of what a particular dimension may encode. 

To analyze the latent space, we use $\psi_{w2}$ (Eq.~\ref{eq:softmax}) as the corresponding embedding vectors and perform T-SNE visualization of the latent $\bm{z}$, similar to what Discover~\cite{sileo2019mining} does using the softmax weight at the final prediction layer. The complete T-SNE result can be found in Appendix~\ref{supp:entire-z2c-mapping}. What we observe is an emerging hierarchical pattern, in addition to proximity. That is, while synonymous markers are clustered as expected, semantically related clusters are often closer. Fig.~\ref{fig:tsne-crop} shows the top left corner of the T-SNE result.
%Here we crop the top left corner of the T-SNE result in Fig.~\ref{fig:tsne-crop} as an example. 
We can see that the temporal connectives and senses are located in the top left corner. According to their coupled markers, we can recover the semantic of these latent $\bm{z}$: preceding ($z_{27}$), succeeding ($z_{25}$, $z_{22}$, $z_{16}$) and synchronous ($z_{15}$) form nearby but separated clusters. 

From \emph{z2m} mapping, we can take a step further to analyze the correlation between markers learned by DMR. Table \ref{tab:m2z} shows the top 2 corresponding clusters of three randomly sampled markers. We can observe correlations between markers like polysemy and synonym.

\subsection{Understanding Entanglement}
\label{sec:exp:discourse}
Labeling discourse relations is challenging since some of them can correlate, and discern the subtleties can be challenging. For example,
% \emph{Cause} can correlate with \emph{Restatement} because we tend to explain reasons by restating it with more details; 
\emph{List} strongly correlates with \emph{Conjunction} and the two are hardly distinguishable. 

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.39\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/num_correct.pdf}
         \caption{}
         \label{fig:rel_he:num_correct}
    \end{subfigure}
    \begin{subfigure}[t]{0.59\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/rel_acc.pdf}
         \caption{}
         \label{fig:rel_he:rel_acc}
    \end{subfigure}
    \caption{Human Evaluation. Figure~(a) shows numbers of reasonable relations in top-3 predictions. Figure~(b) shows the accuracy for each of the top-3 predictions evaluated by annotations or human, respectively.}
    \label{fig:rel_he}
\end{figure}

DMR is trained to predict a \emph{distribution} of markers, thus we expect its hidden state to capture the distribution of relations as well even when the multi-sense labels are scarce.
We drew 100 random samples and ask a researcher to check whether each of the corresponding top-3 predictions is reasonable and give a binary justification. Fig.~\ref{fig:rel_he:num_correct} shows that a considerable amount of 64\% examples have two or more relations evaluated as reasonable in top-3 predictions, much higher than 2.3\% multi-sense labels in PDTB2. This suggests that one way to improve upon the lack of multi-sense annotation is to use DMR to provide candidates for the annotators. For these samples, we also inspect annotator agreement in PDTB2 (Fig.~\ref{fig:rel_he:rel_acc}). While the trend is consistent with what DMR reports, it also validates again that the PTDB2 annotators under-labeled multi-senses.
% We perform a human evaluation in Appendix~\ref{supp:human_eval} to check whether each of the corresponding top-3 predictions is reasonable. The results show that a considerable amount of 64\% examples have two or more relations evaluated as reasonable in top-3 predictions, much higher than 2.3\% multi-sense labels in PDTB2.

To gain a deeper understanding of relation correlation, we rank the sentence pairs according to the entropy of relation prediction, a higher entropy suggests more model uncertainty, namely more confusion.

We use the top-3 predictions of the 20 highest entropy examples to demonstrate highly confusing discourse relations as shown in Fig.~\ref{fig:rel_confusion}. The accumulated joint probability of paired relations on these examples is computed as weights in the confusion matrix. The statistics meet our expectation that there exist specific patterns of confusion. For example, asynchronous relations are correlated with causal relations, while another type of temporal relations, synchronous ones are correlated with conjunction. A complete list of these high entropy examples is listed in Appendix~\ref{supp:human-eval}.

To conclude, while we believe explicit relation labeling is still useful, it is incomplete without also specifying a distribution. As such, DMR's $h_z$ or the distribution of markers are legitimate alternatives to model inter-sentence discourse.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/rel_pp.pdf}
    \caption{Confusion on Discourse Relations. We use entropy as the metric for filtering most confusing examples. We use the top-3 predictions of the 20 most confusing examples to show the entanglement between relations. We use accumulated $p(r_i)\cdot p(r_j)$ as weights for a pair of relations $r_i, r_j$. Note that implausible predictions are suppressed to ignore model errors.}
    \label{fig:rel_confusion}
\end{figure}

\subsection{Case Study on Specific Examples}

\begin{table*}[]
    \centering
    \scalebox{0.9}{
    \begin{tabular}{|p{5cm}|p{5cm}|c|c|c}
        \toprule
        $s_1$ & $s_2$ & markers & relations \\ \midrule
        Rather, they tend to have a set of two or three favorites & Sometimes, they'll choose Ragu spaghetti sauce & \makecell{because\_of\_this\\ therefore\\ for\_example\\ for\_instance} & \makecell{Contingency.Cause \\ Expansion.Instantitation} \\\hline
        
        It just makes healthy businesses subsidize unhealthy ones and gives each employer less incentive to keep his workers healthy & the HIAA is working on a proposal to establish a privately funded reinsurance mechanism to help cover small groups that can't get insurance without excluding certain employees & \makecell{because\_of\_this\\ conversely\\ therefore\\ in\_contrast} & \makecell{Contingency.Cause\\ Comparison.Contrast} \\\hline
        
        The Hart-Scott filing is then reviewed and any antitrust concerns usually met & Typically, Hart-Scott is used now to give managers of target firms early news of a bid and a chance to use regulatory review as a delaying tactic & \makecell{although \\ though \\ besides \\ also} & \makecell{Comparison.Concession \\ Expansion.Conjunction} \\
        \bottomrule
    \end{tabular}
    }
    \caption{Case Study on Marker Ambiguity and Discourse Relation Entanglement.}
    \label{tab:cases}
\end{table*}

==> tables/commonsense.tex <==
\begin{table*}[t!]
    \centering
    \scalebox{0.9}{
    \begin{tabular}{cccccccc}
    \toprule
        Data & Models & isAfter & isBefore & HinderedBy & xWant & xNeed & xReact \\\midrule
        \multirow{2}{*}{ATOMIC~\cite{sap2019atomic}} & BASE & - & - & - & 64.2& 59.8& 62.7 \\
         & DMV & - & - & - & \textbf{67.1} & \textbf{62.6} & \textbf{68.3} \\\hline
        \multirow{2}{*}{ATOMIC2020~\cite{hwang2021comet}} & BASE & 54.8 & 65.0 & 62.9 & 63.1 & 61.5 & 64.2 \\
         & DMV & \textbf{65.9} & \textbf{74.3} & \textbf{71.5} & \textbf{68.3} & \textbf{63.7} & \textbf{69.4} \\ \hline
        \multirow{2}{*}{COMET~\cite{hwang2021comet}} & BASE & 56.0 & 63.4 & 64.7 & 63.5 & 60.6 & 63.3 \\
         & DMV & \textbf{65.3} & \textbf{71.2} & \textbf{73.6} & \textbf{67.8} & \textbf{62.5} & \textbf{68.0}
        \\
    \bottomrule
    \end{tabular}
    }
    \caption{Few-shot Commonsense Relation Modeling}
    \label{tab:fewshot-disc}
\vspace{-10pt}
\end{table*}

% \begin{table}[]
%     \centering
%     \scalebox{0.9}{
%     \begin{tabular}{cccc}
%     \toprule
%         & SWAG & HellaSwag & SMR \\ \midrule
%         BASE$^\diamond$ & 0.762 & 0.469 & 0.500 \\
%         BASE-ATOMIC & 0.650 & 0.419 & 0.502 \\
%         COMET-ATOMIC & 0.422 & 0.278 & 0.350 \\
%         DMV-max & 0.469 & 0.470 & 0.674 \\
%         DMV-avg & 0.528 & 0.527 & 0.691 \\
%         BASE + DMV-avg & \textbf{0.833} & \textbf{0.656} & \textbf{0.766} \\
%         Human & \underline{0.880} & \underline{0.945} & \underline{0.975} \\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Zero-shot Commonsense Reasoning. The BASE$^\diamond$ model here refers to a RoBERTa large model with results replicated based on the implementation in~\cite{zhou2020evaluating}.}
%     \label{tab:com-inf}
% \end{table}

\begin{table}[t]
    \centering
    \scalebox{0.9}{
    \begin{tabular}{cccc}
    \toprule
        & SWAG & HellaSwag & SMR \\ \hline\midrule
        Human & 0.880 & 0.945 & 0.975 \\ \hline
        BASE$^\diamond$ & 0.762 & 0.469 & 0.500 \\
        DMV-max & 0.469 & 0.470 & 0.674 \\
        DMV-avg & 0.528 & 0.527 & 0.691 \\ \hline
        GPT2-ATOMIC & 0.422 & 0.278 & 0.350 \\
        BASE-ATOMIC & 0.650 & 0.419 & 0.502 \\
        BASE + DMV-avg & \textbf{0.833} & \textbf{0.656} & \textbf{0.766} \\ \hline
        \bottomrule
    \end{tabular}
    }
    \caption{Zero-shot Commonsense Reasoning. The BASE$^\diamond$ model here refers to a RoBERTa large model with results replicated based on the implementation in~\cite{zhou2020evaluating}. GPT2-ATOMIC is the COMET model~\cite{hwang2021comet} based on a GPT2XL trained on ATOMIC commonsense triples. BASE-ATOMIC is a roberta model trained on ATOMIC commonsense triples with extra verbalization and grammar check for adaptation to natural text.}
    \label{tab:com-inf}
\vspace{-10pt}
\end{table}


==> tables/linear-prob-cls.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{lcccccccc}
    \toprule
        Models & MR &CR &SUBJ &MPQA &SST2 &TREC &MRPC &AVG \\\midrule\hline
        \multicolumn{8}{c}{Unsupervised Models} \\\midrule
        Vanilla BERT (AVG) & 78.66 & 86.25 & 94.37 & 88.66 & 84.40 & 92.80 & 69.54 & 84.94 \\
        Vanilla BERT (CLS) & 78.68 & 84.85 & 94.21 & 88.23 & 84.13 & 91.40 & 71.13 & 84.66 \\
        SimCSE-unsup (bert-base) & 81.18 & 86.46 & 94.45 & 88.88 & 85.50 & 89.80 & 74.43 & 85.81 \\
        SimCSE-unsup (bert-large) & 85.13 & 89.48 & 95.05 & 89.31 & 90.44 & 88.80 & 74.20 & 87.49 \\ 
        SimCSE-unsup (roberta-base) & 81.10 & 86.92 & 92.77 & 86.74 & 86.60 & 83.80 & 73.51 & 84.49 \\ 
        SimCSE-unsup (roberta-large) & 82.74 & 87.87 & 93.66 & 88.22 & 88.58 & 92.00 & 69.68 & 86.11 \\
        cpt-text(S) & 87.1 & 90.1 & 94.9 & 88.3 & 91.8 & 95.2 & 71.6 & 88.4 \\
        \hline\hline
        \multicolumn{8}{c}{Self-supervised Models (Discourse Marker Data)} \\\midrule
        Discovery (LSTM) & 82.60 & 87.40 & 94.50 & 91.00 & 85.20 & 93.40 & 76.60 & 86.90 \\
        Discovery (roberta-base) & 85.20 & 89.88 & 94.85 & 85.58 & 89.62 & 88.40 & 72.64 & 86.60 \\
        DMV (bert-base) & 81.77 & 86.92 & 94.63 & 88.52 & 86.82 & 89.80 & 73.86 & 86.05 \\
        DMV (bert-large) & 85.62 & 89.25 & 95.50 & 89.88 & 91.32 & 93.20 & 76.87 & 88.81 \\
        DMV (roberta-base) & 84.98 & 90.62 & 94.64 & 88.17 & 90.61 & 88.60 & 74.78 & 87.49 \\
        DMV (roberta-large) & 88.61 & 93.14 & 96.21 & 89.07 & 93.47 & 92.00 & 74.72 & 89.60 \\
        \hline\hline
        \multicolumn{8}{c}{Supervised  Models (Natural Language Inference Data)} \\\midrule
        SBERT-base & 83.64 & 89.43 & 94.39 & 89.86 & 88.96 & 89.60 & 76.00 & 87.41 \\
        SBERT-large & 84.88 & 90.07 & 94.52 & 90.33 & 90.66 & 87.4 & 75.94 & 87.69 \\ 
        cpt-text(S) & 87.3 & 91.0 & 94.6 & 90.5 & 91.4 & 95.0 & 75.6 & 89.3 \\
        SimCSE-sup (bert-base) & 82.69 & 89.25 & 94.81 & 89.59 & 87.31 & 88.40 & 73.51 & 86.51 \\
        SimCSE-sup (bert-large) & 85.44 & 90.81 & 95.25 & 90.26 & 90.33 & 90.60 & 76.29 & 88.43 \\ 
        SimCSE-sup (roberta-base) & 85.01 & 92.00 & 94.05 & 89.84 & 91.27 & 88.00 & 75.65 & 87.97 \\ 
        SimCSE-sup (roberta-large) & 88.12 & 92.37 & 95.11 & 90.49 & 92.75 & 91.80 & 76.64 & 89.61 \\ \hline
        \bottomrule
    \end{tabular}
    \caption{Main results for Linear Probe Classification}
    \label{tab:linear-prob-cls}
\end{table*}
